No Cost Likelihood Manipulation at Test Time for Making Better Mistakes in Deep Networks

There has been increasing interest in building deep hierarchy-aware classifiers that aim to quantify and reduce the severity of mistakes, and not just reduce the number of errors. The idea is to exploit the label hierarchy (e.g., the WordNet ontology) and consider graph distances as a proxy for mistake severity. Surprisingly, on examining mistake-severity distributions of the top-1 prediction, we find that current state-of-the-art hierarchy-aware deep classifiers do not always show practical improvement over the standard cross-entropy baseline in making better mistakes. The reason for the reduction in average mistake-severity can be attributed to the increase in low-severity mistakes, which may also explain the noticeable drop in their accuracy. To this end, we use the classical Conditional Risk Minimization (CRM) framework for hierarchy-aware classification. Given a cost matrix and a reliable estimate of likelihoods (obtained from a trained network), CRM simply amends mistakes at inference time; it needs no extra hyperparameters and requires adding just a few lines of code to the standard cross-entropy baseline. It significantly outperforms the state-of-the-art and consistently obtains large reductions in the average hierarchical distance of top-$k$ predictions across datasets, with very little loss in accuracy. CRM, because of its simplicity, can be used with any off-the-shelf trained model that provides reliable likelihood estimates.

==> matrixproduct.tex <==
\begin{tikzpicture}
\node (A) [text width=2.1cm] {$
    \begin{bmatrix}
        0 & 1 & 2 & 2 \\
        1 & 0 & 2 & 2 \\
        2 & 2 & 0 & 1 \\
        2 & 2 & 1 & 0 \\
    \end{bmatrix}
$};

\node (cross) [right=0cm of A] {$\times$};

\node (v) [text width=1cm, right=0.05cm of cross] {$\begin{array}{c}
    \cellcolor{green!35} 0.35 \\
    \cellcolor{green!25} 0.25 \\
    \cellcolor{green!38} 0.38 \\
    \cellcolor{green!2} 0.02 \\
  \end{array}$};
  
\node (equal) [right=0cm of v] {$=$};

\node (p) [text width=1cm, right=0.05 of equal] {$\begin{array}{c}
    \cellcolor{green!20} 1.05 \\
    \cellcolor{green!22} 1.15 \\
    \cellcolor{green!24} 1.22 \\
    \cellcolor{green!34} 1.58 \\
  \end{array}$};
\end{tikzpicture}
